CatFree3D: Category-agnostic 3D Object Detection with Diffusion

Image-based 3D object detection is widely employed in applications such as autonomous vehicles and robotics, yet current systems struggle with generalisation due to complex problem setup and limited training data. We introduce a novel pipeline that decouples 3D detection from 2D detection and depth prediction, using a diffusion-based approach to improve accuracy and support category-agnostic detection. Additionally, we introduce the Normalised Hungarian Distance (NHD) metric for an accurate evaluation of 3D detection results, addressing the limitations of traditional IoU and GIoU metrics. Experimental results demonstrate that our method achieves state-of-the-art accuracy and strong generalisation across various object categories and datasets.

==> sec/01_intro_v0.tex <==
\section{Introduction}

Image-based 3D object detection systems are designed to identify and localise objects in three-dimensional space from input images. These systems play a critical role in applications like autonomous vehicles and robotics.

Unlike other vision tasks (\ie 2D detection, segmentation,  depth estimation) where unified models demonstrate In this section, we show the model's versatility with various inputs, including 2D prompts alone or in combination with reference images and 3D data. We test it on images from COCO and nerfstudio datasets with novel object categories, showcasing the model's strong generalisation ability.remarkable robustness and generalisation ability~\cite{reis2023real, depthanything, kirillov2023segment}, existing monocular 3D detection models~\cite{brazil2023omni3d, li2024unimode} are typically applied to specific domains and categories. These models often struggle to generalise to unseen categories and adapt to new tasks.

One reason for the limited performance is the relatively small number of available 3D detection datasets, primarily due to the high cost of dataset annotation. As illustrated in \cref{fig: annotation}, human annotators typically have to manually adjust the 9 DoF bounding box and ensure its projection matches the object across multiple views, which is a labour-intensive process. This makes it particularly challenging to gather a substantial amount of data necessary for training a foundation model. 

We explore alternative approaches to training a 3D detector from scratch.
Since 3D detection is closely related to various tasks such as 2D detection, depth estimation, and object pose estimation, we can approach it differently. 
Rather than treating 3D detection as an isolated problem and training a model that demands extensive 3D labelling, we can leverage conditioning signals from these related tasks. This approach helps mitigate the need for large-scale training data.

In our approach, we assume that 2D detection and object depth are provided by external sources. We then focus on estimating the in-plane translation, dimensions, and orientation of the 3D bounding box with the given information.


Another factor that limits the generalisation ability of existing models is their reliance on category labels.  Many models use categorical information as priors or training labels to enhance 3D box estimations~\cite{nie2020total3dunderstanding, brazil2023omni3d, chen2016monocular}. 
While this helps in learning 3D boxes, it limits the model's ability to generalise to new categories, which can be problematic for real-world applications due to the cost and effort involved in labelling new data and retraining for specific objects.

To address this, we adopt a category-agnostic approach, meaning we do not use category information during training or inference. This approach sets our work apart from previous 3D object detection models, which are typically constrained to specific categories and scenarios—either indoor or outdoor—based on their training data. Our experimental results show that our model can effectively generalise to novel object categories and datasets.


Another limitation of the generalisation of the 3D detection model is the proposal generation process. The standard 3D detection approach involves generating 2D/3D proposals and estimating the 3D bounding box of the object based on each proposal. These proposals can be class-specific 3D proposals filtered with semantic and location priors~~\cite{chen20153d, chen2016monocular}, 2D object proposals from Reginal Proposal Network (RPN)~\cite{brazil2023omni3d, nie2020total3dunderstanding}, learnable queries~\cite{wang2022detr3d}.  
While these proposals enable better 3D box regression, they introduce additional network parameters to learn and add domain-specific hyperparameters that may not generalise well to other scenarios. 
We propose to simplify this process by using only random noise as proposals and apply conditional denoising diffusion to gradually recover the target box.
% Depending on the task, our model can either collaborate with 2D detectors for 3D detection with classification or be utilised for applications like obstacle detection, where identifying the object's location is more critical than determining its class.

In developing our novel 3D detection method, we discovered that conventional metrics, such as Intersection over Union ($IoU$) and Generalised IoU ($GIoU$), struggle to evaluate 3D detection results accurately for non-overlapping and enclosing cases, which occurs more frequently for thin and small objects.
% especially regarding bounding box orientation, position, and small object dimensions. 
To address these limitations, we propose a new metric called Normalised Hungarian Distance ($NHD$). This metric first finds an optimal one-to-one assignment between the corners of the ground truth and predicted 3D bounding boxes, then calculates the Euclidean distance between the corresponding corners. This approach allows $NHD$to provide a more detailed and precise evaluation of 3D object detection tasks.

To summarise, our contributions are threefold:
\textbf{First}, we introduce a category-agnostic 3D object detection method that generates 3D bounding boxes conditioned on vision prompts, removing reliance on category-specific priors.
\textbf{Second}, we develop this method with a novel conditional diffusion pipeline, which gradually recover the target box from random noise.
\textbf{Third}, we propose the Normalised Hungarian Distance ($NHD$) metric for a more precise evaluation of 3D detection results.
As a result, our method achieves state-of-the-art accuracy in 3D object detection without needing category information and demonstrates strong generalisation to new categories and datasets.

% We use diffusion to convert a deterministic regression task to a stochastic probabilistic process

% Application 

==> sec/01_intro_v1.tex <==
\section{Introduction}

% existing approach cite 123
% good -> applications
% bad -> train 1 app, cannot transfer to another
% why: require category prior 
% limitation -> motivate : remove category prior

% propose
% setup, assumption
% justify the assumption:
% 1. 2d detection models are widely available
% 2. during training, it's okay to assume GT depth available, during testing, we can use monodepth
% (minor: data efficient)

% with this setup, propose diffusion-based pipeline.


What is 3D object detection? why do we need 3D det? While it is useful in ABC applications for XYZ, in this work, we focuses on developing a category-agnostic 


3DoD method that is strongly beneficiall to a specific application, assisting 3D object detection ground truth labelling, which is crutial in ground truth dataset creation.

% Existing object detection GT labelling pipeline: the current 3D obj detection datasets are labelled by first acquiring some initialisation in the form of 3D bounding boxes, followed by a human adjustment of all 9 DoF for the 3D box based on checking the 2D projection of the target 3D box on a second view. 

Two widely adopted 3D box initialisation options. The first options is to take advantage of off-shelf 3DoD methods such as XXX. However, most 3DoD methods require pre-estimated category-specific size priors as input, thus are constrained to a number of pre-defined categories.

To label unseen categories, the second choice to init a 3D box by leveraging 2D object proposals and depth of the objects, where 2D detection proposals can come from GT 2D labelling or category-agnostic 2D detection systems, and object depth can be triangulated via a pair of images of the object (image pairs are usually avaialble as the final labelling results need to be checked and refined by human annotaters via the projection of the 3D box on the image pairs).
While this initialisation are more flexiable when facing various categories, the orientation component in the 3D init is often inaccurate, requring a time consuming human adjustment process. 

These limitations of XXX and XXX motivate us to develop a novel categories-agnostic 3DoD method to reduce the cost of 3D object detection dataset labelling.

Our key idea is to leverage the diffusion process, which progressively refines a noisy 3D bouding box proposal towards its ground truth, conditioned on an input image, a 2D detection bounding box, and the object depth, assuming 2D bounding box proposals and object depth available -- same to the second 3D bound box initialisation option mentioned above.

If the metric is a thing, mention it in this paragraph.
If the metric is a thing, mention it in this paragraph.
If the metric is a thing, mention it in this paragraph.
If the metric is a thing, mention it in this paragraph.
If the metric is a thing, mention it in this paragraph.
\TODO{}

To summarise, our contributions are threefold:
First, we introduce the first category-agnostic 3D object detection method. 
Second, we propose a novel diffusion-based pipeline to achieve category-agnostic 3D object detection. 
Third, We propose a new metric for 3D object detection that is effective in scenarios where $IoU_{3D}$ fails to rank predictions precisely. \zirui{rephrase this after finishing metric paragraph}
As a result, our method achieves state-of-the-art 3D object detection accuracy without needing pre-defined category priors, reducing the cost of 3D object detection dataset significantly.



==> sec/01_intro_v2.tex <==
\section{Introduction}
Image-based 3D object detection systems are designed to identify and localise objects in three-dimensional space from input images. These systems play a critical role in applications like autonomous vehicles and robotics.





% need to rewrite para 2-6

% P2-3 start from existing method, 
% arch: joint 2d 3d and depth prediction.
% while used in many apps, has two limitations
% 1. class-dependent
% 2. slow training

% P4: key idea need to change to decouple, diffusion/generation is just an approach
% P5: decouple benefit 1: class-free
% P6: decouple benefit 2: faster training


Recent developments in deep learning has significant advanced 3D object detection research~\cite{chen2016monocular, simonelli2019disentangling, zhang2021objects, nie2020total3dunderstanding}. While these methods have been widely adopted in applications above, these 3D detection methods remain largely domain-specific and are limited to a number of object categories.

Several works have proposed expanding 3D detection systems to handle more categories by building larger datasets~\cite{brazil2023omni3d} and learning domain-specific parameters to unify indoor and outdoor scenes~\cite{li2024unimode}. \ul{However, these methods are intrinsically limited to pre-defined categories.} As a result, models trained on a specific set of categories struggle to generalise to unseen categories. This limitation arises because these methods require category information such as pre-estimated priors or class labels, constraining them to pre-defined categories.

We propose a category-agnostic 3D object detection method to address this limitation. 
\ul{Our key idea involves generating a 3D bounding box from a noisy initial proposal, conditioning on a number of vision prompts.}
This generation process is performed by a denoising network inspired by diffusion literature~\cite{ho2020denoising, song2020denoising}. 

Specifically, the noisy proposal is initialised from a normal distribution, and vision prompts include the image of the target object, a 2D detection bounding box, and the depth of the target.
\ul{By decoupling both the initial proposal and the vision prompts from specific categories, our method eliminates the reliance on category-specific priors}, thereby enhancing the flexibility and generality of 3D object detection.

% We further propose to improve the training efficiency by leveraging readily available 2D bounding box proposals and object depth. 
% Unlike common 3D detection methods, which requires a costly training process as they usually need to learn to predict 2D and 3D bounding boxes and depth jointly, 
% We, instead, propose to untie the 2D bound box prediction and depth prediction from the 3D object detection task. 
% During training, we take advantage of ground truth labels of 2D bounding boxes and object depths. During inference, we leverage powerful modern 2D detection and monocular depth prediction networks. As will be shown in our experiment section, this design choice leads to a much more data efficient training process and reducing training time significantly.

By using readily available 2D bounding box proposals and object depth information, our method also enhance training efficiency. Unlike conventional 3D detection methods that require a joint training of 2D and 3D bounding boxes and depth, we suggest decoupling the 2D bounding box prediction and depth prediction from the 3D object detection task. By utilising ground truth labels for training and modern 2D detection and monocular depth networks for inference, we achieve a more data-efficient training process and significantly reduce training time.

In addition to utilising category-agnostic noisy proposals and vision prompts, diffusion-based methods can generate \textit{arbitrary} number of predictions for a \textit{single} target due to their stochastic nature.
We leverage this by estimating multiple 3D bounding boxes for one target, assigning a confidence score to each, and selecting the most confident one, which boost the performance.

During developing our novel 3D detection method, we discovered that conventional metrics, such as Intersection over Union (IoU) and Generalised IoU (GIoU), struggle to evaluate 3D detection results accurately for non-overlapping and enclosing cases, which occurs more frequently for thin and small objects.
To address these limitations, we propose a new metric called Normalised Hungarian Distance (NHD). This metric first finds an optimal one-to-one assignment between the corners of the ground truth and predicted 3D bounding boxes, then calculates the Euclidean distance between the corresponding corners. This approach allows NHD to provide a more detailed and precise evaluation of 3D object detection tasks.

% To summarise, our contributions are threefold:
% \textbf{First}, we introduce the first category-agnostic 3D object detection method. 
% \textbf{Second}, we develop this method with a novel diffusion pipeline, which predicts a 3D bounding box given an image, a 2D bounding box and the depth of a target object.
% \textbf{Third}, we propose a new metric for 3D object detection that provides a more detailed and precise evaluation in 3D object detection tasks than conventional IoU and GIoU.

To summarise, our contributions are threefold: \textbf{First}, we introduce a category-agnostic 3D object detection method that generates 3D bounding boxes conditioned on vision prompts, removing reliance on category-specific priors. \textbf{Second}, we design a novel diffusion-based method to recover box parameters from an arbitrary number of noisy proposals while estimate the confidence of each prediction.
\textbf{Third}, we propose the Normalised Hungarian Distance (NHD) metric for a more precise evaluation of 3D detection results.

As a result, our method achieves state-of-the-art accuracy in 3D object detection without needing category information and demonstrates strong generalisation to new categories and datasets.






% We also demonstrate that our method, while using ground truth depth during training, are able to utilise various sources of depth during inference. 

% The rest of this paper is arranged as follows: sec xxx related work, sec xxx our diffusion based method, sec xxx the new metric, sec xxx experiment and finally sec xxx conclude.




% existing approach cite 123
% good -> applications
% bad -> train 1 app, cannot transfer to another
% why: require category prior 
% limitation -> motivate : remove category prior

% propose
% setup, assumption
% justify the assumption:
% 1. 2d detection models are widely available
% 2. during training, it's okay to assume GT depth available, during testing, we can use monodepth
% (minor: data efficient)

% with this setup, propose diffusion-based pipeline.

==> sec/02_related_v0.tex <==
\section{Related Work}
Object detection has been extensively studied, resulting in a vast body of literature. This section focuses on 2D and 3D object detection from a single image, covering both classical approaches and recently developed diffusion-based methods.



\subsection{Single Image 2D Object Detection}
\boldstart{Classical}
2D object detection approaches include "two-stage detectors"~\cite{girshick2015fast, ren2015faster} that follow a coarse-to-fine manner and "one-stage detectors"~\cite{carion2020end, reis2023real, ren2015faster, liu2016ssd} that directly estimate objects from the feature backbone. 
Category-agnostic 2D detection models are conceptually similar to our approach in that they avoid using category information. These models learn to differentiate generic objects from the image background using low-level visual cues~\cite{zitnick2014edge, o2015learning} or using supervision from bounding box labels~\cite{maaz2022class, jaiswal2021class, kim2022learning}.



\boldstart{Diffusion-based}
DiffusionDet~\cite{chen2023diffusiondet} was the first to apply diffusion to detection tasks, progressively refining noisy 2D boxes towards the target objects.
In visual perception tasks, DiffusionDet~\cite{chen2023diffusiondet} was the first to apply box diffusion for 2D object detection from a single RGB image. 
However, instead of learning objectness like these methods, we focus on mapping 2D boxes to 3D boxes by leveraging visual cues from the input image.
\zirui{is there any other diffusion based 2d detection methods?}







\subsection{Single Image 3D Object Detection}
\boldstart{Classical}
Monocular 3D object detectors predict 3D cuboids from a single input image. Depending on the dataset domain, certain models are tailored for outdoor scenes for self-driving~\cite{chen2016monocular, huang2022monodtr, ranasinghe2024monodiff, liu2021ground, ma2019accurate, mousavian20173d, reading2021categorical, wang2022probabilistic, mousavian20173d}, while others are specifically designed for indoor environments~\cite{nie2020total3dunderstanding, huang2018cooperative, tulsiani2018factoring, kulkarni20193d}. Additionally, some studies~\cite{rukhovich2022imvoxelnet, brazil2023omni3d, li2024unimode} have explored integrating both indoor and outdoor datasets during training. 
These methods often use category labels for supervision~\cite{brazil2023omni3d, huang2022monodtr, li2024unimode, liu2021ground}, require category information as a prior for initialisation or as input~\cite{nie2020total3dunderstanding, brazil2023omni3d, ranasinghe2024monodiff}, or focus on specific scenes and object categories with strong assumptions about the predictions' dimensions or orientation~\cite{simonelli2019disentangling, yan2024monocd, chen2016monocular, mousavian20173d}. This reliance on category and scenario-specific knowledge limits their generalisation to in-the-wild scenes and novel categories. 
In contrast, our approach does not use category information during training or inference, focusing solely on predicting 3D bounding boxes. This allows the model to be used for novel objects that were not present during training.



\boldstart{Diffusion-based}
For 3D object detection, Zhou \emph{et al.}~\cite{zhou2023diffusion} introduced diffusion of 5 DoF Bird’s Eye View boxes as proposals for detection from point clouds. Diffusion-SS3D~\cite{ho2024diffusion} employs diffusion for semi-supervised object detection in point clouds, denoising object size and class labels. DiffRef3D~\cite{kim2023diffref3d} and DiffuBox~\cite{chen2024diffubox} apply diffusion to refine proposals/coarse boxes for 3D object detection from point clouds.
MonoDiff~\cite{ranasinghe2024monodiff} uses Gaussian Mixture Models to initialise the dimensions and poses of 3D bounding boxes, recovering the target boxes through diffusion conditioned on an image.
Unlike these approaches, which assume an initial distribution or proposals for the diffusing box parameters~\cite{ranasinghe2024monodiff, chen2024diffubox}, limited DoFs for box orientation and dimensions~\cite{kim2023diffref3d, chen2024diffubox}, or diffuse only partial parameters~\cite{ho2024diffusion, ranasinghe2024monodiff}, our model initialise box parameters with random noise to diffuse. By conditioning the model on an image and a 2D box, our model recovers the in-plane translations, 3 dimensions, and 3 DoF rotations of the 3D box through diffusion.











% \subsection{3D Object Detection}

% \textbf{Image-based 3D Object Detection}
% 3D object detection can be categorised based on the input signals, such as images, point clouds, depth, etc. 
% Image-based 3D detection approaches~\cite{chen2016monocular, brazil2023omni3d, nie2020total3dunderstanding, wang2022detr3d, xu2023nerf, rukhovich2022imvoxelnet} take one or multiple images as input and estimate the 3D object boxes together with class prediction. 
% These methods typically require a fixed number of anchors or 2D/3D proposals to be generated at the first stage and estimate 3D boxes based on these proposals. 
% Mono3D~\cite{chen2016monocular} generates 3D proposals with priors on semantics, shape and location. Cube R-CNN~\cite{brazil2023omni3d} uses the 2D Reginal Proposal Network (RPN) and estimates offsets of 3D boxes to the 2D proposals on the image plane. 
% DETR3D~\cite{wang2022detr3d} proposes to use learnable object queries and make a box prediction for each query.
% It is also possible to make 3D box estimation based on 2D detection results
% \cite{ku2019monocular, nie2020total3dunderstanding}.
%  By contrast, our method generates random 3D proposals and learns to transform these proposals to the target box through diffusion. The number of proposals is arbitrary and can be different during training and inference.
%  Note that we use 2D boxes as prompts instead of proposals in our network, i.e. the number of predictions we make is independent of the number of 2D box prompts. 

% \subsection{Image-based 3D Object Detection}
% Given the RGB images and corresponding camera parameters, the 3D object detection models~\cite{chen2016monocular, brazil2023omni3d, nie2020total3dunderstanding, wang2022detr3d, xu2023nerf, rukhovich2022imvoxelnet} estimate 3D bounding boxes and classes for objects. 









% This task is an ill-posed problem due to inherent scale ambiguity when estimating the object's depth. Cube R-CNN~\cite{brazil2023omni3d} introduces 'virtual depth' to account for variations in camera intrinsic, but the ambiguity in 3D remains. DDMP-3D~\cite{wang2021depth} uses depth maps conditioned on images to learn depth-aware features. AutoShape~\cite{liu2021autoshape} employs vehicle CAD models to impose geometric constraints on monocular detection. 
% Pseudo-LiDAR is also commonly used to boost the detection performance~\cite{park2021pseudo, xu2023mononerd}.
% These methods typically require a fixed number of anchors or 2D/3D proposals to be generated at the first stage and estimate 3D boxes based on these proposals. 
% Mono3D~\cite{chen2016monocular} generates 3D proposals with priors on semantics, shape and location. Cube R-CNN~\cite{brazil2023omni3d} uses the 2D Reginal Proposal Network (RPN) and estimates offsets of 3D boxes to the 2D proposals on the image plane. 
% It is also possible to make 3D box estimation based on 2D detection results
% \cite{mousavian20173d, ku2019monocular, nie2020total3dunderstanding}.
%  By contrast, our method generates random 3D proposals and learns to transform these proposals to the target box through diffusion. 
% Note that our model takes 2D boxes as prompts instead of proposals. Thus for each 2D box, we can make an arbitrary number of predictions.
% A recent diffusion-based monocular 3D detection approach, MonoDiff~\cite{ranasinghe2024monodiff}, shares a similar concept of estimating the 3D bounding box through the denoising diffusion. However, unlike our method, precomputed Gaussian Mixture Models are required to model the distribution for parameter initialisation and diffusion is not applied to box translation.
% In our model, we decouple depth estimation from other box parameters and learn to recover these parameters given specific object depth and intrinsic values. During testing, we accept depth and intrinsic data from various sources.
% 3DiffTection~\cite{xu20243difftection} uses
% \zirui{what is the diff between this paragraph and the last paragraph?}



% Diffusion models~\cite{ho2020denoising, sohl2015deep, song2019generative, song2020score} has demonstrated remarkable results in various fields including vision tasks~\cite{harvey2022flexible, yang2023diffusion, ho2022video}, natural language processing~\cite{austin2021structured, gong2023diffuseq, li2022diffusion, yu2022latent}, and multimodal data generation~\cite{avrahami2022blended, ramesh2022hierarchical, rombach2021high, poole2022dreamfusion, zhang2023adding}.
% \textbf{Diffusing 3D representations}: 
% Beyond 2D images, diffusion models have also been applied to various 3D representations including point clouds~\cite{luo2021diffusion, vahdat2022lion, melas2023pc2}, 3D RGB and density grids~\cite{ntavelis2023autodecoding}, and 3D feature grids~\cite{karnewar2023holodiffusion} for tasks such as shape generation and view synthesis. 
% The 3D bounding box, as a lightweight 3D representation of an object, has been explored for diffusion with different parameterisations. 
% Zhou \emph{et al.}~\cite{zhou2023diffusion} applied diffusion to generate 5 DoF Bird’s Eye View (BEV) boxes. Diffusion-SS3D~\cite{ho2024diffusion} denoises object size and class label. 
% A concurrent work DiffuBox~\cite{chen2024diffubox} applies 7 DoF bounding box diffusion to box refinement task, conditioned on point cloud. 
% In our model, we diffuse 9 DoF bounding boxes.
% \textbf{Diffusion for Visual Perception}:
% Additionally, diffusion has been utilised for tasks like image segmentation~\cite{amit2021segdiff, chen2023generalist} and human pose estimation~\cite{gong2023diffpose, holmquist2023diffpose}.




% Unlike these approaches that are conditioned on point clouds, our approach is conditioned on an image and a 2D prompt.


==> sec/02_related_v1.tex <==
\section{Related Work}
Object detection has been extensively studied, resulting in a vast body of literature. This section focuses on 2D and 3D object detection from a single image, covering both classical approaches and recently developed diffusion-based methods.



\subsection{Single Image 2D Object Detection}
\boldstart{Classical}
2D object detection approaches include "two-stage detectors"~\cite{girshick2015fast, ren2015faster} that follow a coarse-to-fine manner and "one-stage detectors"~\cite{carion2020end, reis2023real, ren2015faster, liu2016ssd} that directly estimate objects from the feature backbone. 
Category-agnostic 2D detection models are conceptually similar to our approach in that they avoid using category information. These models learn to differentiate generic objects from the image background using low-level visual cues~\cite{zitnick2014edge, o2015learning} or using supervision from bounding box labels~\cite{maaz2022class, jaiswal2021class, kim2022learning}.



\boldstart{Diffusion-based}
DiffusionDet~\cite{chen2023diffusiondet} was the first to apply diffusion models to object detection tasks, progressively refining noisy 2D boxes towards the target objects. While DiffusionDet focuses on box diffusion for 2D object detection from a single RGB image, our approach differs by focusing on mapping 2D boxes to 3D boxes, utilising visual cues from the input image.
% \zirui{is there any other diffusion based 2d detection methods?}







\subsection{Single Image 3D Object Detection}
\boldstart{Classical}
Monocular 3D object detectors predict 3D cuboids from a single input image. Depending on the dataset domain, some models are tailored for outdoor scenes in self-driving applications~\cite{chen2016monocular, huang2022monodtr, ranasinghe2024monodiff, liu2021ground, ma2019accurate, mousavian20173d, reading2021categorical, wang2022probabilistic, mousavian20173d}, while others are designed for indoor environments~\cite{nie2020total3dunderstanding, huang2018cooperative, tulsiani2018factoring, kulkarni20193d}. Additionally, some studies~\cite{rukhovich2022imvoxelnet, brazil2023omni3d, li2024unimode} have explored integrating both indoor and outdoor datasets during training.

These methods often rely on category labels for supervision~\cite{brazil2023omni3d, huang2022monodtr, li2024unimode, liu2021ground}, require category information for initialization or as input~\cite{nie2020total3dunderstanding, brazil2023omni3d, ranasinghe2024monodiff}, or focus on specific scenes and object categories with strong assumptions about the dimensions or orientation of the predictions~\cite{simonelli2019disentangling, yan2024monocd, chen2016monocular, mousavian20173d}. This dependence on category and scenario-specific knowledge limits their generalization to novel categories and in-the-wild scenes. In contrast, our approach does not use category information during training or inference, focusing solely on predicting 3D bounding boxes. This enables the model to generalize to novel objects not seen during training.



\boldstart{Diffusion-based}
For 3D object detection, Zhou \emph{et al.}~\cite{zhou2023diffusion} introduced diffusion of 5 DoF Bird’s Eye View boxes for detection from point clouds. 
Diffusion-SS3D~\cite{ho2024diffusion} employs diffusion for semi-supervised object detection in point clouds, denoising object size and class labels. 
DiffRef3D~\cite{kim2023diffref3d} and DiffuBox~\cite{chen2024diffubox} apply diffusion to refine proposals/coarse boxes for 3D object detection from point clouds. \zirui{all point cloud}

MonoDiff~\cite{ranasinghe2024monodiff} uses Gaussian Mixture Models to initialise the dimensions and poses of 3D bounding boxes, recovering the target boxes through diffusion conditioned on an image.

Unlike these approaches, which assume an initial distribution or proposals for the diffusing box parameters~\cite{ranasinghe2024monodiff, chen2024diffubox}, limited degrees of freedom for box orientation and dimensions~\cite{kim2023diffref3d, chen2024diffubox}, or predict only partial parameters~\cite{ho2024diffusion, ranasinghe2024monodiff}, our model initialise box parameters with random noise. By conditioning our model on image-related prompts, our method effectively recovers a 3D box up to scale.











% \subsection{3D Object Detection}

% \textbf{Image-based 3D Object Detection}
% 3D object detection can be categorised based on the input signals, such as images, point clouds, depth, etc. 
% Image-based 3D detection approaches~\cite{chen2016monocular, brazil2023omni3d, nie2020total3dunderstanding, wang2022detr3d, xu2023nerf, rukhovich2022imvoxelnet} take one or multiple images as input and estimate the 3D object boxes together with class prediction. 
% These methods typically require a fixed number of anchors or 2D/3D proposals to be generated at the first stage and estimate 3D boxes based on these proposals. 
% Mono3D~\cite{chen2016monocular} generates 3D proposals with priors on semantics, shape and location. Cube R-CNN~\cite{brazil2023omni3d} uses the 2D Reginal Proposal Network (RPN) and estimates offsets of 3D boxes to the 2D proposals on the image plane. 
% DETR3D~\cite{wang2022detr3d} proposes to use learnable object queries and make a box prediction for each query.
% It is also possible to make 3D box estimation based on 2D detection results
% \cite{ku2019monocular, nie2020total3dunderstanding}.
%  By contrast, our method generates random 3D proposals and learns to transform these proposals to the target box through diffusion. The number of proposals is arbitrary and can be different during training and inference.
%  Note that we use 2D boxes as prompts instead of proposals in our network, i.e. the number of predictions we make is independent of the number of 2D box prompts. 

% \subsection{Image-based 3D Object Detection}
% Given the RGB images and corresponding camera parameters, the 3D object detection models~\cite{chen2016monocular, brazil2023omni3d, nie2020total3dunderstanding, wang2022detr3d, xu2023nerf, rukhovich2022imvoxelnet} estimate 3D bounding boxes and classes for objects. 









% This task is an ill-posed problem due to inherent scale ambiguity when estimating the object's depth. Cube R-CNN~\cite{brazil2023omni3d} introduces 'virtual depth' to account for variations in camera intrinsic, but the ambiguity in 3D remains. DDMP-3D~\cite{wang2021depth} uses depth maps conditioned on images to learn depth-aware features. AutoShape~\cite{liu2021autoshape} employs vehicle CAD models to impose geometric constraints on monocular detection. 
% Pseudo-LiDAR is also commonly used to boost the detection performance~\cite{park2021pseudo, xu2023mononerd}.
% These methods typically require a fixed number of anchors or 2D/3D proposals to be generated at the first stage and estimate 3D boxes based on these proposals. 
% Mono3D~\cite{chen2016monocular} generates 3D proposals with priors on semantics, shape and location. Cube R-CNN~\cite{brazil2023omni3d} uses the 2D Reginal Proposal Network (RPN) and estimates offsets of 3D boxes to the 2D proposals on the image plane. 
% It is also possible to make 3D box estimation based on 2D detection results
% \cite{mousavian20173d, ku2019monocular, nie2020total3dunderstanding}.
%  By contrast, our method generates random 3D proposals and learns to transform these proposals to the target box through diffusion. 
% Note that our model takes 2D boxes as prompts instead of proposals. Thus for each 2D box, we can make an arbitrary number of predictions.
% A recent diffusion-based monocular 3D detection approach, MonoDiff~\cite{ranasinghe2024monodiff}, shares a similar concept of estimating the 3D bounding box through the denoising diffusion. However, unlike our method, precomputed Gaussian Mixture Models are required to model the distribution for parameter initialisation and diffusion is not applied to box translation.
% In our model, we decouple depth estimation from other box parameters and learn to recover these parameters given specific object depth and intrinsic values. During testing, we accept depth and intrinsic data from various sources.
% 3DiffTection~\cite{xu20243difftection} uses
% \zirui{what is the diff between this paragraph and the last paragraph?}



% Diffusion models~\cite{ho2020denoising, sohl2015deep, song2019generative, song2020score} has demonstrated remarkable results in various fields including vision tasks~\cite{harvey2022flexible, yang2023diffusion, ho2022video}, natural language processing~\cite{austin2021structured, gong2023diffuseq, li2022diffusion, yu2022latent}, and multimodal data generation~\cite{avrahami2022blended, ramesh2022hierarchical, rombach2021high, poole2022dreamfusion, zhang2023adding}.
% \textbf{Diffusing 3D representations}: 
% Beyond 2D images, diffusion models have also been applied to various 3D representations including point clouds~\cite{luo2021diffusion, vahdat2022lion, melas2023pc2}, 3D RGB and density grids~\cite{ntavelis2023autodecoding}, and 3D feature grids~\cite{karnewar2023holodiffusion} for tasks such as shape generation and view synthesis. 
% The 3D bounding box, as a lightweight 3D representation of an object, has been explored for diffusion with different parameterisations. 
% Zhou \emph{et al.}~\cite{zhou2023diffusion} applied diffusion to generate 5 DoF Bird’s Eye View (BEV) boxes. Diffusion-SS3D~\cite{ho2024diffusion} denoises object size and class label. 
% A concurrent work DiffuBox~\cite{chen2024diffubox} applies 7 DoF bounding box diffusion to box refinement task, conditioned on point cloud. 
% In our model, we diffuse 9 DoF bounding boxes.
% \textbf{Diffusion for Visual Perception}:
% Additionally, diffusion has been utilised for tasks like image segmentation~\cite{amit2021segdiff, chen2023generalist} and human pose estimation~\cite{gong2023diffpose, holmquist2023diffpose}.




% Unlike these approaches that are conditioned on point clouds, our approach is conditioned on an image and a 2D prompt.


==> sec/03_method_v1.tex <==

\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\textwidth]{images/model.pdf}
    \caption{\textbf{Training Pipeline.} 
At each training step, we add noise to the xy-plane translation, dimensions, and rotations of the ground truth 3D box to generate
$N$ independent proposals at a random time step
t. We then estimate the transformations needed to recover the ground truth box from these proposals using a denoising decoder. This decoding process is conditioned on the RGB image and a 2D prompt for the target object. The loss is calculated as the Chamfer distance between the
$N$ predictions, weighted by their confidence, and the ground truth 3D box.}
    \label{fig: training model}
\end{figure*}

\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\textwidth]{images/inference.pdf}
    \caption{\textbf{Inference Pipeline.} During inference, our model decodes $N_{eval}$ randomly initialised $N_{eval}$ proposals at certain depth(s) into $N_{eval}$ predictions and select the box with highest confidence as the final prediction.}
    \label{fig: inference model}
\end{figure*}


\section{Method}
\subsection{Preliminary}
\textbf{Diffusion Models}
% \zirui{
% 1. No need to mention $\beta$ and this equation. They are irrelavant to 3D detection. 
% 2. You need to mention high-level conditioning idea, then mention our conditioning a little bit, then refer to sec.xxx for more details in prompt/conditioning.
% 3. Use a simple high level function should be enough.
% }
Diffusion Probabilistic Models ~\cite{ho2020denoising} learns the reverse process of a predefined stochastic diffusion process that gradually transforms a simple initial distribution (e.g., Gaussian noise) into a complex data distribution.
The forward diffusion process can be described as

describes the process of adding Gaussian noise $\mathbf{\epsilon}$ to data progressively over $T$ time steps. 
The backward process is 

This denoise process can be modelled as a $f_\theta(\mathbf{x}_t, t)$ to predict $\mathbf{x}_0$ through a neural network. 
% which is formulated as 
% \begin{equation}
%     q(\mathbf{x}_t | \mathbf{x}_{t-1}) = \mathcal{N}(\mathbf{x}_t; \sqrt{1 - \beta_t} \mathbf{x}_{t-1}, \beta_t \mathbf{I})
% \end{equation}
% where $\beta_t$ is a hyperparameter representing the variance schedule and $\mathbf{x}_t$ is the data at time step $t$. In our case, $\mathbf{x}_t$ represents a 3D box.
We train a model $f_\theta(\mathbf{x}_t, t)$ to predict $\mathbf{x}_0$ through a neural network. 
% the objective can be written as
% \begin{equation}
% \label{eq: diffusion1}
%     L_{DM} = \mathbb{E}_{t\sim[1, T], \mathbf{\epsilon} \sim \mathcal{N}(0, 1), \mathbf{x}_0} \mathcal{L}(f_\theta(\mathbf{x}_t, t), \mathbf{x}_0)
% \end{equation}
During inference, the model reverses the forward process, denoising $\mathbf{x}_t$ back to $\mathbf{x}_0$, with the trained model and update rules~\cite{ho2020denoising, song2020denoising}. 
Similar to prompts for image diffusion~\cite{rombach2021high, zhang2023adding}, we model conditional distributions by adding conditional signals $\mathbf{c}$ to $f_\theta$, which include an image $I$, a 2D box prompt $\mathbf{B}_{2D}^*$ and the object depth $z^*$. The training objective can be written as
\begin{equation}
\label{eq: diffusion2}
    L_{CDM} = \mathbb{E}_{t\sim[1, T], \mathbf{\epsilon} \sim \mathcal{N}(0, 1), \mathbf{x}_0} \mathcal{L}(f_\theta(\mathbf{x}_t, t, \mathbf{c}), \mathbf{x}_0)
\end{equation}
Details about the prompt conditioning mechanism and loss function $\mathcal{L}(.)$ are in \cref{sec: prompt} and \cref{sec: loss} respectively.
We choose DDIM sampling~\cite{song2020denoising} to achieve efficient sampling with fewer steps.
% The reverse process can be expressed as:
% \begin{equation}
%     p_\theta(\mathbf{x}_{t-1} | \mathbf{x}_t) = \mathcal{N}(\mathbf{x}_{t-1}; \mu_\theta(\mathbf{x}_t, t), \sigma_t^2 \mathbf{I})
% \end{equation}

\subsection{Model Overview}
% We address the problem of monocular 3D object detection, with given 2D prompts and object depth. 

Given a single RGB image $I$, a 2D bounding box of an object $\mathbf{B}_{2D}^*$, known object depth $z^*$, and camera intrinsic $K$, our objective is to estimate the xy-plane translation, dimensions and orientation of the 3D box that encloses the object.
% determine the smallest 3D bounding box with arbitrary orientation that fully encloses the object. 
% \zirui{Add some math symbols here to elaborate the statment above.}

    \boldstart{Training:} During training, we randomly select one object from all objects shown on an image and generate $N$ independent noisy box proposals by adding noise to the box parameters through forward diffusion, and train a model $f_\theta$ to recover the target box from noisy boxes. 

\boldstart{Inference:} During Inference, for each query object, we initialise a random 3D box with Gaussian noise at a certain depth and denoise the box to obtain $M$ predictions through DDIM diffusion. Note that the number of proposals during training and inference can be different. We select the box with the highest confidence score as the final prediction.

\subsection{Box Parameterisation and Normalisation}
We represent each 3D bounding box with 12 parameters. The coordinates $[u, v]$ denote the projection of the object's centre on the image plane, assuming known camera intrinsics. The depth of the object's centre is indicated by $z \in \mathbb{R}+$. The dimensions $\mathbf{d}$ of the 3D bounding box in metres are given by $[w, h, l] \in \mathbb{R}+^3$. The object's 6D rotation relative to the camera pose of the input image is represented by $\mathbf{p} \in \mathbb{R}^6$~\cite{zhou2019continuity}. 

Before introducing noise to the 3D object box, we first normalise the parameters of the box to the range $[-1, 1]$ and then scale them to $[-S, S]$, where $S$ is the signal-to-noise ratio of the diffusion process. We then apply Gaussian noise to the box parameters. The coordinates $[u, v]$ are normalised with respect to the image dimensions $[H, W]$.
% and the depth $z$ is normalised against a predefined depth range. 
Each dimension of the bounding box is normalised against a predefined size range. Since the parameters for 6D rotation naturally fall within the range $[-1, 1]$, no additional processing is required.



\subsection{Prompts Conditioning and Decoder}
\label{sec: prompt}
The denoising decoder $f_\theta(\mathbf{x}_t, t, \mathbf{c})$ estimates the target $\mathbf{x}_0$ by learning the transformation from noisy box parameters $\mathbf{x}_t$ towards $\mathbf{x}_0$ at time step $t$. 
The conditioning signal $\mathbf{c}$ includes the image feature $F$, a 2D bounding box $\mathbf{B}_{2D}^*$, the object depth $z^*$, and camera intrinsics $(f_x, f_y)$. 
The image feature $F$ is obtained by encoding the input image $I$ with a pre-trained Swin Transformer~\cite{liu2021swin}. 
We then extract image features inside the region of the 2D box prompt $F_{RoI}$ and use a cross-attention layer~\cite{vaswani2017attention} with the 2D prompt to obtain $F_{atten}$, which is then concatenated with $F_{RoI}$.
The 2D bounding box $\mathbf{B}_{2D}^*$ is described by the centre of the box along with its height and width on the image plane, i.e. $[u_{2d}, v_{2d}, w_{2d}, h_{2d}]$. 
We further unproject the height and width of the 2D box to the 3D via
\begin{equation}
    (w_{3d}, h_{3d}) = (w_{2d} * \frac{z}{f_x}, h_{2d} * \frac{z}{f_y})
\end{equation}
and concat $[u_{2d}, v_{2d}, w_{3d}, h_{3d}]$ with the image features [$F_{RoI}$, $F_{atten}$] to obtain the final conditioning signal $\mathbf{c}$. 

Our decoder uses the noisy $\mathbf{x}_t$ as proposals, along with conditioning signals $\mathbf{c} = [F_{RoI}, F_{atten}, u_{2d}, v_{2d}, w_{3d}, h_{3d}]$ and time step $t$, to estimate the box transformations from the proposals toward the target $\mathbf{x}_0$ while also estimating the confidence of each prediction. 
Following the approach of ~\cite{chen2023diffusiondet, sun2021sparse}, our decoder is structured with 6 cascading stages, reusing the same decoding block where each stage's input proposals are the output of the previous block. 
In each decoding block, we concatenate the positionally encoded $\mathbf{x}_t$ with the conditioning signals $\mathbf{c}$, passing this combination through MLPs to generate a single feature. This feature is linearly transformed with the timestep embedding and processed through MLPs to produce the 3D transformation estimates. These 3D transformations are then applied to the proposals to yield the final predictions $\mathbf{B}_{3D}^{pred}$. Additionally, we use the feature obtained before applying the timestep transformation to estimate the uncertainty $\mu$ for each prediction via MLPs. The confidence score is derived by mapping the uncertainties $\mu$ from the range $(0, \infty)$ to $(0, 1)$ using $e^{-\mu}$.

\subsection{Losses}
\label{sec: loss}
Unlike conventional diffusion models~\cite{ho2020denoising, song2020denoising} that are trained with $l_2$ loss, we use loss that allows noncanonical 3D box estimation.
Inspired by Cube R-CNN~\cite{brazil2023omni3d}, our losses consist of a 3D loss and an uncertainty regularisation. 

For each prediction, the 3D loss $\mathcal{L}_{3D}$ is computed as the chamfer distance between the corners of the ground truth 3D box $C_{gt}$ and the corners of the predicted boxes $C_{pred}$.
\begin{equation}
    \mathcal{L}_{3D} = \sum_{c_1 \in C_{pred} }\min_{c_2 \in C_{gt}} \|c_1 - c_2\|_1 + \sum_{c_2 \in C_{gt}} \min_{c_1 \in C_{pred}} \|c_2 - c_1\|_1
\end{equation}
We weight each prediction by their predicted confidence score $e^{-\mu}$ and add the predicted uncertainty for regulariation, to prevent the uncertainty from being too large.
% \zirui{elaborate chamfer distance}

The training objective is written as 
\begin{equation}
    \mathcal{L} = e^{-\mu} \mathcal{L}_{3D} + \lambda_{\mu} \mu
\end{equation}
where $\lambda_{\mu}$ is a hyperparameter for weighting.


\subsection{New Metric: normalised Hungarian Distance}
\label{sec: model_metric}

\begin{figure*}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{images/simulate.pdf}
    \caption{Comparison Between $nHD$, $IoU_{3D}$ and $GIoU_{3D}$. }
    \label{fig: simulate}
\end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/metric.pdf}
    \caption{\textbf{Comparison of $IoU_{3D}$ and $nHD$ in a practical case.} For thin objects like mirrors, monocular detection usually fails to estimate depth correctly, leading to $IoU_{3D}=0$. $nHD$ can reflect the error in this case.}
    \label{fig: metric}
\end{figure}

Intersection-over-union of 3D object bounding box ($IoU_{3D}$) is a commonly used metric for evaluating 3D object detection performance~\cite{brazil2023omni3d, rukhovich2022imvoxelnet, nie2020total3dunderstanding}. While it is advantageous for being scale-invariant, the metric fails to indicate the closeness of the prediction when two boxes do not overlap. It becomes a significant problem for thin and small objects (i.e. mirrors, televisions) since a small estimation error can cause the prediction to be off from the ground truth. One example is shown in \cref{fig: metric}. New metrics like generalised intersection-over-union ($GIoU$)~\cite{rezatofighi2019generalized} have been proposed to address this problem. However, it cannot measure how well the box centre, scale and orientation align with the ground truth in some cases as shown in ~\cref{fig: simulate}.

We propose a new metric, normalised Hungarian Distance ($nHD$), which keeps the scale-invariant property while avoiding the problem in certain cases shown in ~\cref{fig: simulate}. The $nHD$ between two boxes is computed as
\begin{equation}
    nHD(C^{pred}, C^{gt}) = \frac{1}{\|\mathbf{d}_{gt}\|_2} \min_{\sigma \in S_n} \sum_{i=1}^n \|a_i - b_{\sigma(i)}\|_2
\end{equation}
where $C^{pred} = \{a_1, a_2, \ldots, a_n\}$ is the corners of the predicted 3D box and $C^{gt} = \{b_1, b_2, \ldots, b_n\}$ is the corners of the ground truth box. $S_n$ represents all permutations of $\{1, 2, \ldots, n\}$. To make the metric invariant to the object scale, we normalise the distance by the length of the space diagonal of the ground truth box $\|\mathbf{d}_{gt}\|_2$.


==> sec/03_method_v2.tex <==
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\textwidth]{images/model.pdf}
    \caption{\textbf{Training Pipeline.} 
At each training step, we add noise to the xy-plane translation, dimensions, and rotations of the ground truth 3D box to generate
$N$ independent proposals at a random time step
t. We then estimate the transformations needed to recover the ground truth box from these proposals using a denoising decoder. This decoding process is conditioned on the RGB image and a 2D prompt for the target object. The loss is calculated as the Chamfer distance between the
$N$ predictions, weighted by their confidence, and the ground truth 3D box.
}
    \label{fig: training model}
\end{figure*}

\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\textwidth]{images/inference.pdf}
    \caption{\textbf{Inference Pipeline.} During inference, our model decodes $N_{eval}$ randomly initialised $N_{eval}$ proposals at a certain depth(s) into $N_{eval}$ predictions and selects the box with the highest confidence as the final prediction.}
    \label{fig: inference model}
\end{figure*}
















\section{Method}
% Given a single RGB image $I$, a 2D bounding box of an object $\mathbf{B}_{2D}^*$, known object depth $z^*$, and camera intrinsic $K$, our objective is to estimate the xy-plane translation, dimensions and orientation of the 3D box that encloses the object. \zirui{why need * here?}
% \zirui{xy-plane translation appears to be too acute here, I know what you mean, but `position' fits better here to me.}

% We formulate the 3D box estimation task as a conditional diffusion process~\cite{ho2020denoising}, progressively refining the target box parameters from Gaussian noise. \zirui{this is great!}

% In the forward diffusion process, Gaussian noise is added incrementally to the box parameters over $T$ time steps until they are completely noisy. During training, we randomly sample a time step $t \in [1, T]$ to obtain noisy parameters $\mathbf{x}_t$ and train a neural network model, $f_\theta(\mathbf{x}_t, t)$, to predict the original box parameters $\mathbf{x}_0$:
% \begin{equation}
%     f_\theta(\mathbf{x}_t, t)  \rightarrow \mathbf{x}_0
% \end{equation}
% During inference, the model reverses the forward process, denoising $\mathbf{x}_T$ back to $\mathbf{x}_0$ using the trained model $f_\theta$ and specific update rules~\cite{ho2020denoising, song2020denoising}.

% Similar to prompts used for image diffusion~\cite{rombach2021high, zhang2023adding}, we
% parameterise the input image, 2D box, object depth and camera intrinsics as a conditioning signal $\mathbf{c}$, and model conditional distributions of box parameters. Consequently, the denoising model $f_\theta$ can be rewritten as
% \begin{equation}
%     f_\theta(\mathbf{x}_t, t, \mathbf{c}) \rightarrow \mathbf{x}_0.
% \end{equation}


Given an image $I$, a 2D bounding box of an object $\mathbf{B}_{2D}$, object depth $z$, and camera intrinsics $K$, our objective is to estimate the centre, 3D dimensions and orientation of a 3D box that tightly encloses the object. 

We formulate this task as a conditional diffusion process~\cite{ho2020denoising}, progressively recovering a target box from Gaussian noise, conditioned on multiple prompts.

Let us consider a general diffusion setup first -- in the forward diffusion process, Gaussian noise is incrementally added to a variable $\mathbf{x}_0$ over $T$ time steps until it follows a normal distribution. 
During backward diffusion, the noise-free variable $\mathbf{x}_0$ can be recovered from its noisy version $\mathbf{x}_t$ using a neural network
% In the backward denoising process, we use a network $f_\theta$ to progressively recover the variable $\mathbf{x}_0$ from a noisy state $\mathbf{x}_t$:
\begin{equation}
    f_\theta(\mathbf{x}_t, t)  \rightarrow \mathbf{x}_0,
    \label{eq:general_diffusion}
\end{equation}
where $t \in [1, T]$ denotes a diffusion step. 


\textit{In our 3D object detection context, we consider $\mathbf{x}_0$ the parameters of a 3D box}.

To adapt the general diffusion process to this vision-based 3D detection setup, we consider a conditional diffusion process
\begin{equation}
\label{eq: 2}
    f_\theta(\mathbf{x}_t, t, \mathbf{c}) \rightarrow \mathbf{x}_0,
\end{equation}
where
% \begin{equation}
%     \mathbf{c} = g(I, \mathbf{B}_{2D}, z, K)
% \end{equation}
$\mathbf{c}$
is the conditional signal containing the information of the input image $I$, a 2D detection box $\mathbf{B}_{2D}$, the object depth $z$ and camera intrinsics $K$. 
This conditional diffusion process is similar to diffusion-based text-to-image generative tasks~\cite{rombach2021high, zhang2023adding}, where the conditional signal is typically text descriptions.

In the following section, we begin by introducing the parameterisation of 2D and 3D bounding boxes in \cref{sec: box_parameter}. Next, we discuss the assembly of our vision prompts in \cref{sec: prompt}. We then explain how to predict a 3D bounding box using our conditional diffusion process in \cref{sec:xxx}, followed by a description of how we utilise the generative properties of diffusion networks to predict multiple proposals and their associated confidence levels. Finally, we outline our training and inference processes in \cref{sec:xxx} and \cref{sec:xxx}.















\subsection{Box Parameterisation}
\label{sec: box_parameter}
We represent each 3D bounding box with 12 parameters. 
The coordinates $[u, v]$ denote the projection of the object's centre on the image plane, assuming known camera intrinsics. 
The depth of the object's centre is indicated by $z \in \mathbb{R}+$. 
The dimensions $\mathbf{d}$ of the 3D bounding box in metres are given by $[w, h, l] \in \mathbb{R}+^3$. 
The object's rotation relative to the camera pose of the input image is represented by the continuous 6D allocentric rotation $\mathbf{p} \in \mathbb{R}^6$~\cite{zhou2019continuity}. Excepting from object depth $z$ which we assume is given as input, our data for diffusion is the remaining 11 box parameters
% \zirui{how to define the position of a box? a certain corner or the centre of a box? the position is a function of z. The relationship between p and z should be specified clearly.}
\begin{equation}
    \mathbf{x}_0 = [u, v, w, h, l, \mathbf{p}].
\end{equation}

Before introducing noise to the 3D box parameters, we first normalise the parameters of the box to the range $[-1, 1]$ and then scale them to $[-S, S]$, where $S$ is the signal-to-noise ratio of the diffusion process. 
We then apply Gaussian noise to the box parameters. The coordinates $[u, v]$ are normalised with respect to the image dimensions $[H, W]$.
% and the depth $z$ is normalised against a predefined depth range. 
Each dimension of the bounding box is normalised against a predefined size range. 
Since the parameters for 6D rotation naturally fall within the range $[-1, 1]$, no additional processing is required.




\subsection{Prompts Conditioning and Decoder}
\label{sec: prompt}
\zirui{I'll just call this denoising network}
The denoising decoder $f_\theta(\mathbf{x}_t, t, \mathbf{c})$ estimates the target $\mathbf{x}_0$ by learning the transformation from noisy box parameters $\mathbf{x}_t$ towards $\mathbf{x}_0$ at time step $t$. 
The conditioning signal $\mathbf{c}$ is derived from the image $I$, a 2D bounding box $\mathbf{B}_{2D}$, the object depth $z$, and camera intrinsics $K$:
\begin{equation}
\mathbf{c} = g(I, \mathbf{B}_{2D}, z, K),
\end{equation}
where the function $g(\cdot)$ serves as an encoding function.
% where
% \begin{equation}
% \mathbf{c} = [F_{RoI}, F_{atten}, u_{2d}, v_{2d}, w_{3d}, h_{3d}]
% \end{equation}
We first encode the input image $I$ with a pre-trained Swin Transformer~\cite{liu2021swin} to obtain multi-scale feature maps $F$. 
We then extract local image features inside the region of the 2D box prompt $F_{RoI}$ and use a cross-attention layer~\cite{vaswani2017attention} with the 2D prompt to obtain $F_{atten}$.

The 2D bounding box $\mathbf{B}_{2D}$ is described by the centre of the box along with its height and width on the image plane, i.e. $[u_{2d}, v_{2d}, w_{2d}, h_{2d}]$. 
We further unproject the height and width of the 2D box to the 3D via
\begin{equation}
    (w_{3d}, h_{3d}) = (w_{2d} \frac{z}{f_x}, h_{2d} \frac{z}{f_y}), 
\end{equation}
where $f_x$ and $f_y$ are the focal lengths from the intrinsics $K$.
By concatenating the transformed box prompt and image features, the final conditioning signal $\mathbf{c}$ can be written as
\begin{equation}
\mathbf{c} = [F_{\text{RoI}}, F_{\text{attn}}, u_{2d}, v_{2d}, w_{3d}, h_{3d}].
\end{equation}
% \zirui{specify fxfy and K}

% Our decoder uses the noisy $\mathbf{x}_t$ as proposals, along with conditioning signals and time step $t$, to estimate the box transformations from the proposals toward the target $\mathbf{x}_0$ while also estimating the confidence of each prediction. 
After obtaining the conditioning $\mathbf{c}$, the decoder $f_\theta$ estimates the box transformation from proposals $\mathbf{x}_t$ towards $\mathbf{x}_0$.
During decoding, we first positional encode~\cite{tancik2020fourier} $\mathbf{x}_t$ and concatenate it with the conditioning signals $\mathbf{c}$ to obtain a single feature.
This feature is linearly transformed with the timestep embedding and processed through MLPs to produce the 3D transformation estimates. These 3D transformations are then applied to the proposals to yield the final prediction $\mathbf{\hat{x}}$.




\subsection{Multiple Proposals and Confidence}
In the original diffusion model, each forward step involves denoising a single $\mathbf{x}_t$ to $\mathbf{x}_0$ using the decoder $f_\theta$. However, in practice, the expressiveness of $f_\theta$ can sometimes be insufficient for transforming difficult samples to $\mathbf{x}_0$. To alleviate this issue, we allow multiple $\mathbf{x}_t$ samples, i.e., $\{\mathbf{x}_t^i|i=1 ... N\}$, to be fed into $f_\theta$, and make N estimations $\{\mathbf{\hat{x}}^i|i=1 ... N\}$ along with their uncertainties $\{\mu^i|i=1 ... N\}$. 
% Therefore, \cref{eq: 2} can be rewritten as
% \begin{equation}
%     f_\theta(\mathbf{x}_t^i, t, \mathbf{c}) \rightarrow \mathbf{x}_0,
% \end{equation}
When computing the loss, by weighing the loss of predictions according to their uncertainties, the model can focus more on the predictions it is confident about.

To estimate the timestep-independent confidence score for each prediction, we add a branch $f_\phi$
\begin{equation}
f_\phi(c, x_t) \rightarrow \mu.
\end{equation}
The confidence score is then derived by mapping the uncertainty $\mu$ from the range $(0, \infty)$ to $(0, 1)$ through $e^{-\mu}$.











\subsection{Training}
\label{sec:training}

For each forward step during training, we randomly select one object from all objects shown on an image and generate $N$ independent noisy box proposals by adding noise to the box parameters through forward diffusion. 
We sample a timestep $t$ and train a model $f_\theta$ to recover the target box parameters from noisy ones. 
The training objective can be written as
% \begin{equation}
% \label{eq: diffusion2}
%     L_{CDM} = \mathbb{E}_{t\sim[1, T], \mathbf{\epsilon} \sim \mathcal{N}(0, 1), \mathbf{x}_0} \sum_{i=1}^N \mathcal{L}(f_\theta(\mathbf{x}_t^i, t, \mathbf{c}), \mathbf{x}_0).
% \end{equation}

\begin{equation}
\label{eq: diffusion2}
    \sum_{i=1}^N \mathcal{L}(f_\theta(\mathbf{x}_t^i, t, \mathbf{c}), \mathbf{x}_0).
\end{equation}


% The training loss can be written as
% \begin{equation}
% \label{eq: diffusion2}\sum_{i=1}^N \mathcal{L}(f_\theta(\mathbf{x}_t^i, t, \mathbf{c}), \mathbf{x}_0)
% \end{equation}
% and we follow the convention of diffusion training.
Unlike conventional diffusion models~\cite{ho2020denoising, song2020denoising} that are trained with $l_2$ loss, we use loss that allows non-canonical 3D box estimation.
Inspired by Cube R-CNN~\cite{brazil2023omni3d}, our losses consist of a 3D loss and an uncertainty regularisation. 

For each prediction, the 3D loss $\mathcal{L}_{3D}$ is computed as the chamfer distance between the corners of the predicted 3D boxes $C^{pred} = \{a_i| i= 1 ... 8\}$ and the corners of the ground truth boxes $C^{gt} =\{b_i| i= 1 ... 8\}$.
\begin{equation}
\label{eq: cd}
    \mathcal{L}_{3D} = \sum_{a_i \in C^{pred} }\min_{b_i \in C^{gt}} \|a_i - b_i\|_1 + \sum_{b_i \in C^{gt}} \min_{a_i \in C^{pred}} \|b_i - a_i\|_1.
\end{equation}
We weight each prediction by their predicted confidence score $e^{-\mu}$ and regularise the predicted uncertainty $\mu$ with a loss term $\mathcal{L}_{reg}=\mu$ to prevent the uncertainty from being too large.
The full loss term can be written as:
\begin{equation}
    \mathcal{L} = e^{-\mu} \mathcal{L}_{3D} + \lambda_{reg} \mathcal{L}_{reg},
\end{equation}
where $\lambda_{reg}$ is a hyperparameter for weighting.



\subsection{Inference}
During Inference, for each query object, we initialise 3D box parameters $\mathbf{x}_T$ with Gaussian noise and denoise the box to obtain $N_{eval}$ predictions through DDIM diffusion~\cite{song2020denoising}. Note that the number of proposals during training and inference can be different. We select the box with the highest confidence score as the final prediction.




\section{Metric: Normalised Hungarian Distance}
\label{sec: model_metric}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{images/simulate.pdf}
    \caption{\textbf{Comparison Between $NHD$, $IoU_{3D}$ and $GIoU_{3D}$}. By comparing (b) (c) (d) to (a), we found that $NHD$ is sensitive to translation, scale and rotation errors when one box fully encloses the other, whereas $IoU_{3D}$ and $IoU_{3D}$ do not capture these error differences. Comparisons between (e) and (f) to (a) show that $NHD$ and $GIoU_{3D}$ can reflect error differences when there is no overlap. (a) and (g) show that all metrics are scale-invariant. (h) show the values of the metrics when the two boxes fully aligned. }
    \label{fig: simulate}
\end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/metric.pdf}
    \caption{\textbf{Comparison of $IoU_{3D}$ and $NHD$ in a practical case.} For thin objects like mirrors, monocular detection usually fails to estimate depth correctly, leading to $IoU_{3D}=0$. $NHD$ can reflect the error in this case.}
    \label{fig: metric}
\end{figure}

Intersection-over-union of 3D object bounding box ($IoU_{3D}$) is a commonly used metric for evaluating 3D object detection performance~\cite{brazil2023omni3d, rukhovich2022imvoxelnet, nie2020total3dunderstanding}. While it is advantageous for being scale-invariant, the metric fails to indicate the closeness of the prediction when two boxes do not overlap. It becomes a significant problem for thin and small objects (i.e. mirrors, televisions) since a small estimation error can cause the prediction to be off from the ground truth. One example is shown in \cref{fig: metric}. New metrics like generalised intersection-over-union ($GIoU$)~\cite{rezatofighi2019generalized} have been proposed to address this problem. However, it cannot measure how well the box centre, scale and orientation align with the ground truth when one box fully encloses the other one, as shown in ~\cref{fig: simulate}.

% We propose a new metric, normalised Hungarian Distance ($NHD$), which keeps the scale-invariant property while avoiding the problem in certain cases shown in ~\cref{fig: simulate}. The $NHD$ between two boxes is computed as
% \begin{equation}
%     $NHD$(C^{pred}, C^{gt}) = \frac{1}{\|\mathbf{d}_{gt}\|_2} \min_{\sigma \in P_n} \sum_{i=1}^n \|a_i - b_{\sigma(i)}\|_2,
% \end{equation}
% where $C^{pred}$ and $C^{gt}$ are the corners of the predicted box and ground truth box as defined in \cref{eq: cd}. $P_n$ represents all permutations of $\{1, 2, \ldots, n\}$. To make the metric invariant to the object scale, we normalise the distance by the length of the space diagonal of the ground truth box $\|\mathbf{d}_{gt}\|_2$.


We propose a new metric, normalised Hungarian Distance ($NHD$), which maintains scale-invariance while addressing certain issues illustrated in ~\cref{fig: simulate}. The $NHD$ between two boxes is computed as
\begin{equation}
    h(C^{pred}, C^{gt}) \rightarrow P,
\end{equation}
\wenjing{add something}
\begin{equation}
    NHD(C^{pred}, C^{gt}) = \frac{1}{\|\mathbf{d}_{gt}\|_2} \sum_{(i, j) \in P} \|a_i - b_{j}\|_2,
\end{equation}
where $C^{pred}$ and $C^{gt}$ are the corners of the predicted box and ground truth box as defined in \cref{eq: cd}. $P$ is list of tuple contains the corners of the best 1-to-1 mapping that minimises the total Euclidean distance between corner pairs. Algorithm $h$ (\eg linear assignment) is used to obtain the mapping. To make the metric invariant to the object scale, we normalise the distance by the length of the space diagonal of the ground truth box $\|\mathbf{d}_{gt}\|_2$.



% \zirui{$C_{pred}$ and gt should be introduced in the training section. Symbol $S$ has been used for scale.}


==> sec/05_exp_old.tex <==
\section{Experiments}
We tackle the problem of category-agnostic 3D object detection from a single RGB image with a 2D prompt and object depth. We first detail datasets, metrics, model design and implementations in \cref{sec: implementation}. In \cref{sec: main_results}, we compare our approach against various baselines to quantitatively demonstrate the accuracy and generalisation ability. The ablation experiments and applications are in \cref{sec: ablation} and \cref{sec: application} respectively. 


\subsection{Implementation Details}
\label{sec: implementation}
\textbf{Datasets} For training and evaluation, we utilise the Omni3D dataset~\cite{brazil2023omni3d}, which is composed of six datasets\cite{song2015sun}, ARKitScenes~\cite{baruch2021arkitscenes}, Hypersim~\cite{roberts2021hypersim}, Objectron~\cite{ahmadyan2021objectron}, KITTI~\cite{geiger2012we}, and nuScenes~\cite{caesar2020nuscenes}, encompassing both indoor and outdoor environments. For the quantitative tests discussed in \cref{sec: application}, we employ the COCO~\cite{lin2014microsoft} and nerfstudio~\cite{nerfstudio} datasets.

\boldstart{Baselines}  To accurately assess the performance of our 3D detector, it is essential to eliminate errors from sources such as 2D detection and depth estimation. In \cref{sec: main_results}, we assume ground truth 2D boxes and depth are provided for all methods during evaluation. We select Cube R-CNN~\cite{brazil2023omni3d} and Total3DUnderstanding~\cite{nie2020total3dunderstanding} as our primary baselines, as their 3D detection heads can function independently.
Additionally, since the baseline methods require category information, we provide ground truth category labels to their models. 
% In \cref{sec: main2}, we integrate our 3D detection with an off-the-shelf 2D detector and depth estimator to enable comparisons with a broader range of 3D detection approaches~\cite{rukhovich2022imvoxelnet, liu2022petr, wang2022probabilistic, li2024unimode}.

\boldstart{Metrics} In \cref{sec: main_results}, we use $IoU_{3D}$ and $NHD$ as two metrics to evaluate the performance of 3D detectors. 
% In \cref{sec: main2}, we employ Average Precision (AP) over a range of $IoU_{3D}$ thresholds according to \cite{brazil2023omni3d}.

\boldstart{Model}
Our model architecture is built on Detectron2~\cite{wu2019detectron2}. We use the Swin Transformer~\cite{liu2021swin} pre-trained on ImageNet-22K~\cite{deng2009imagenet} as the image feature encoder and freeze all parameters during training. The denoising decoder adopts the iterative architecture in Sparse R-CNN~\cite{sun2021sparse} with 6 blocks, where the predictions from the previous stage are used as the proposals for the next stage. Predictions from each stage are used to compute loss against the ground truth.

\boldstart{Training \& Inference}
We train the model for 270k iterations with a batch size of 16 on 2 A5000 GPUs. 
In comparison, Cube R-CNN is trained on 48 V100 GPUs with a batch size of 192.
We use AdamW optimiser~\cite{kingma2014adam} with a learning rate of $2.5 \times 10^{-5}$ which decays by a factor of 10 at 150k and 200k iterations. During training, we use image augmentation including random horizontal flipping and resizing.
During evaluation, as the proposals are initialised with random noise, the result can vary with different random seeds. To obtain a stable result, experiment results reported in \cref{sec: main_results} and \cref{sec: unseen} are computed by averaging the results of 10 different random seeds. We also analyse the stability of model performance with random seeds in the supplementary material.
\subsection{Performance of 3D Detectors}
\label{sec: main_results}
\begin{figure}[]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/main.pdf}
    \caption{\textbf{Prediction Results on SUN RGB-D test set}. We take 2D boxes and object depths as inputs and estimate the in-plane translations, dimensions and orientations of 3D boxes.}
    \label{fig: main1}
\end{figure}
% As previous approaches either require category information~\cite{brazil2023omni3d, nie2020total3dunderstanding} or make predictions of a certain category~\cite{simonelli2019disentangling}, we take their results for reference only. 
We compare our model with state-of-the-art 3D object detection approaches on 10 common categories for indoor environments following~\cite{brazil2023omni3d}. For baseline models~\cite{brazil2023omni3d, nie2020total3dunderstanding}, we assume ground truth 2D boxes as the oracle 2D detection results and provide category information. In contrast, our method requires 2D boxes only and does not use the category information. Our model uses the depth estimated by \cite{brazil2023omni3d} for a fair comparison.
We introduce a variant of each method that substitutes estimated object depths with ground truth depths. As shown in \cref{table: main}, our approach outperforms the baselines, even with their use of additional category information and dimension priors. The comparison between using predicted depths (upper half of table) and ground truth depths (lower half) highlights that inaccurate monocular depth estimation is a key source of error in monocular 3D detection models.
% The full evaluation of all categories is in the supplementary material.

\begin{table*}[]
\centering
\begin{tabular}{lcccccccccccc}
\hline
\multirow{2}{*}{Methods} &  & \multicolumn{2}{c}{SUN RGB-D}  &  & \multicolumn{2}{c}{OMNI3D\_IN} &  & \multicolumn{2}{c}{OMNI3D\_OUT} &  & \multicolumn{2}{c}{OMNI3D} \\ \cline{3-4} \cline{6-7} \cline{9-10} \cline{12-13} 
                         &  & IoU $\uparrow$           & NHD  $\downarrow$           &  & IoU $\uparrow$               & NHD $\downarrow$        &  & IoU $\uparrow$             & NHD  $\downarrow$           &  & IoU $\uparrow$             & NHD $\downarrow$      \\ \hline
Total3D                  &  & 24.8          & 0.376          &  & -                 & -          &  & -              & -              &  & -               & -        \\
Cube R-CNN               &  & 36.2          & 0.236          &  &                   &            &  & 27.4           & 0.594          &  &                 &          \\
Ours-d                   &  & \textbf{40.2} & \textbf{0.231} &  & \textbf{}         &            &  &                &                &  &                 &          \\ \hline
Total3D*                 &  & 46.6          & 0.184          &  & -                 & -          &  & -              & -              &  & -               & -        \\
Cube R-CNN*              &  & 54.5          & 0.137          &  &                   &            &  & 58.3           & 0.118          &  &                 &          \\
Ours*                    &  & \textbf{61.4} & \textbf{0.114} &  & \textbf{}         &            &  & \textbf{60.2}  & \textbf{0.115} &  & \textbf{}       &      \\ \hline   
\end{tabular}
\caption{\textbf{Comparison to Cube R-CNN~\cite{brazil2023omni3d} and Total3DUnderstanding~\cite{nie2020total3dunderstanding} on Omni3D.} We use ground truth 2D detections and ground truth classes fairly for all methods and report IoU and NHD. Ours-d takes the depth predicted by Cube R-CNN. The * indicates that the ground truth depths are used in the predictions.}
\end{table*}


\subsection{Generalisation on Novel Categories}
\label{sec: unseen}
\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/unseen.pdf}
    \caption{\textbf{Prediction Results on Novel Categories}. We found that the model can generalise well to object categories (such as tables, cabinets, and sofas) that are not present in the training data. }
    \label{fig: unseen}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\columnwidth]{images/unproject.pdf}
%     \caption{\textbf{Unprojection Baseline Visualisation}}
%     \label{fig: unproject}
% \end{figure}
To verify our model's generalisation ability across different objects, we trained it on the SUN RGB-D dataset using 31 out of 38 categories and evaluated it on the remaining categories. Since there are no previous baselines for comparison, we created a simple baseline using axis-aligned 3D boxes to demonstrate the importance of estimating in-plane offsets and box orientation, as well as the effectiveness of our approach. This baseline method takes the 2D box prompt and back-projects it to 3D using the provided depth and focal length. The bounding box orientation is set to match the camera orientation, and the dimension in the z-direction is set to the maximum length of the ground truth bounding box in that direction. 
% A visualisation example of the baseline is shown in \cref{fig: unproject}. 
Results in \cref{table: unseen} and \cref{fig: unseen} show that our approach significantly outperforms this baseline and demonstrates good generalisation ability.
% We further conduct cross-dataset, cross-category tests in \cref{sec: application}.


\begin{table*}[]
\centering
\begin{tabular}{l|l|lllllll|l}
Methods   & Trained on    & sofa & table & cabinet & toilet & bathtub & door & oven & avg. \\ \hline
Unproject & N/A           & 28.2 & 27.1  & 28.6    & 25.6   & 23.9    & 23.6 & 37.2 & 27.7     \\
Ours      & SUN RGB-D & 56.4 & 56.8 & 53.0 & 61.3 & 46.7 & 27.7 & 62.1 & 52.0     
\end{tabular}
\caption{\textbf{Quantatitive Results for novel categories.} We train the model on 31 categories and evaluate it on 7 unseen categories in the SUN RGB-D test set and report $IoU_{3D}$.}
\label{table: unseen}
\end{table*}





\subsection{Discussion}
\label{sec: ablation}

% \todo{show our method is data efficient}

\begin{table}[]
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabular}{l|ll}
SNR & $IoU_{3D}\uparrow$ & $NHD\downarrow$   \\ \hline
1.0 & 57.2  & 0.195   \\
2.0 & 59.8 & 0.177 \\
3.0 & 59.7  & 0.178
\end{tabular}
\caption{Signal-to-noise ratio}
\label{table: snr}
\end{subtable}%
% \end{table}
% \begin{table}[]
\hfill
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabular}{l|ll}
Iter steps &$IoU_{3D}\uparrow$ & $NHD\downarrow$   \\ \hline
1          & 61.19  & 0.1153 \\
3          & 61.23  & 0.1150 \\
5          & 61.28  & 0.1147
\end{tabular}
\caption{Inference iteration steps.}
\label{table: steps}
\end{subtable}
% \end{table}
% \begin{table}[]
\vspace{1cm} % Space between tables
\begin{subtable}[t]{0.45\textwidth}
\centering
% \begin{tabular}{l|ccc}
%             & \multicolumn{3}{c}{$N_{eval}$} \\
% $N_{train}$ & 1        & 10       & 100      \\ \hline
% 1           & 58.1     & 60.2     & 60.2     \\
% 10          & 60.9     & 61.2     & 61.2     \\
% 100         & 61.2     & 61.4     & 61.4    
% \end{tabular}
\begin{tabular}{llccc}
            &  & \multicolumn{3}{c}{$N_{eval}$} \\ \cline{3-5} 
$N_{train}$ &  & 1        & 10       & 100      \\ \hline
1           &  & 58.1     & 60.2     & 60.2     \\
10          &  & 60.9     & 61.2     & 61.2     \\
100         &  & 61.2     & 61.4     & 61.4    
\end{tabular}
\caption{Training and sampling proposals. We report $IoU_{3D}$ 
% \zirui{redo this table}
}
\label{table: props}
\end{subtable}
% \end{table}
% \begin{table}[]
\hfill
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabular}{ll|ll}
$\sigma_{scale}$ & $\sigma_{trans}$ & $IoU_{3D}\uparrow$ & $NHD\downarrow$   \\ \hline
0.00       & 0.00       & 61.4  & 0.114 \\
0.05       & 0.00       & 59.9  & 0.120 \\
0.00       & 0.05       & 56.1  & 0.132 \\
0.05       & 0.05       & 55.2  & 0.135 \\
0.10       & 0.10       & 46.1  & 0.174 
\end{tabular}
\caption{Noise on the 2D prompt}
\label{table: noise}
\end{subtable}
\caption{\textbf{Model Analysis on SUN RGB-D dataset.}}
\end{table}

We conducted model analysis on the 10 common categories in the SUN RGB-D test set to study its performance. Unless otherwise stated, all inferences are run with 10 proposals at a single sampling step.

\boldstart{Signal-to-noise ratio.}
In \cref{table: snr}, we show the influence of the diffusion process's signal-to-noise ratio (SNR). Setting SNR to 2 achieves the highest performance in $IoU_{3D}$ and $NHD$, which is consistent with the observations in other diffusion models for detection~\cite{chen2023diffusiondet, kim2023diffref3d}.

\boldstart{Inference iteration steps.}
During inference, we observed that increasing the number of DDIM sampling steps enhances model performance, albeit at the cost of longer inference times. As shown in \cref{table: steps}, raising the iteration steps from 1 to 5 results in performance gains, which plateau with additional steps.

\boldstart{Training and inference proposals.}
Since we use random noise to initialise proposals, the number of proposals is flexible and can vary between training ($N_{train}$) and inference ($N_{eval}$). \cref{table: props} presents the results for different combinations of $N_{train}$ and $N_{eval}$. We observed that increasing $N_{train}$ enhances model performance, with a cost of larger memory consumption. However, increasing $N_{eval}$ beyond 10 does not yield additional improvement. Consequently, we select $N_{train} = 100$ and $N_{eval} = 10$ for the remaining experiments.

\boldstart{Noise on the 2D prompt.}
We analyse the model's robustness towards noise during inference in \cref{table: noise}. We simulate box noise by applying Gaussian noise to box scales and translations separately.
\cref{table: noise} shows that while the model is robust to noise in box scale and translation, translation errors have a greater impact on accuracy.



% \subsection{Metric Analysis}
% \label{sec: metric}

% As discussed in \cref{sec: model_metric}, we introduce normalized Hungarian Distance ($NHD$) as a new metric for measuring the accuracy of 3D detection. In this section, we highlight the advantages of $NHD$ by comparing it to $IoU_{3D}$ in our experiments. As shown in \cref{fig: metric}, for thin objects like mirrors and televisions, inaccurate depth estimation can easily result in zero overlaps between the ground truth box and the prediction. In these cases, $IoU_{3D}$ cannot effectively rank the quality of predictions. Conversely, $NHD$ provides a reliable reference that correlates with the predicted box's translation, dimension and orientation.

\subsection{Generalisation to various data}
\subsection{Application}
\zirui{rephrase subtitles}
% \subsection{generalisation to various depth sources}
\label{sec: application}
% In this part, we analyse the performance of our model on in-the-wild scenes to demonstrate its generalisation ability for novel object categories and how this model can work under different settings.
% \zirui{should we call this section: generalisation to various depth sources, and call the dataset labelling the actual application?}

In this section, we show the model's versatility with various inputs, including 2D prompts alone or in combination with reference images and 3D data. We test it on images from COCO and nerfstudio datasets with novel object categories, showcasing the model's strong generalisation ability.

\boldstart{2D prompts$\rightarrow$ 3D box projection} 
% \zirui{3D box is good enough, or remove 3D box from all subtitles}
% \boldstart{depth source: random} 
When given only 2D prompts, our model can estimate up-to-scale 3D boxes with projections that align with the objects in the image, even if the provided depth and intrinsics are inaccurate. \cref{fig: coco} shows examples where we set the same depth and camera intrinsics for all objects.

\begin{figure*}[]
    \centering
    \includegraphics[width=0.9\linewidth]{images/coco.pdf}
    \caption{\textbf{Prediction results for in-the-wild objects on COCO dataset with 2D prompt.} We set all objects' focal lengths and depths to the same values. Despite not having accurate depth estimation, the model can predict in-plane translations, orientation, and box dimensions, resulting in a good 2D projection. }
    \label{fig: coco}
\end{figure*}

\boldstart{2D prompt $+$ posed multi-view images $\rightarrow$ 3D box}
% \boldstart{depth source: real depth} 
When multi-view images and camera poses are available, we can resolve depth ambiguity by projecting 3D boxes across different views. Starting with a 2D prompt, we generate 3D box predictions over a range of possible depths from a source view. These boxes are then projected onto other views, and the best match is selected. 
 A notable feature of our model is its ability to generate an arbitrary number of proposals, enabling multiple predictions.
This approach can be incorporated into a 3D box annotation pipeline, significantly improving annotation efficiency, as shown in \cref{fig: annotation}. 

\begin{figure*}[]
    \centering
    \includegraphics[width=0.9\linewidth]{images/annotation.pdf}
    \caption{\textbf{3D Detection Dataset Annotation.} In the original pipeline (left), annotators manually adjust the box until the projection looks correct in each view. We offer an alternative approach, allowing the annotator to select the best box from the candidates generated from our model (right).
    % \zirui{this selection is not easy too. Does the method offer a best prediction?}
    }
    \label{fig: annotation}
\end{figure*}

\boldstart{2D prompt $+$ depth/3D reference $\rightarrow$ 3D box}
% \boldstart{depth source: monoculr depth} 
In many application scenarios, available depth or 3D information can assist in estimating the 3D box using our model.
By using monocular metric depth estimation~\cite{depthanything, piccinelli2024unidepth} and object segmentation~\cite{kirillov2023segment}  models, we can roughly estimate object depths by averaging the depth values within the object mask, facilitating a reliable top-view projection as shown in \cref{fig: monodepth}.
When 3D data (\ie point clouds, CAD models) is available, it can be used to infer object depth, as illustrated in \cref{fig: pcd}.
\begin{figure}[]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/monodepth.pdf}
    \caption{\textbf{Prediction with 2D prompts and metric depth estimation.}
    We infer object depths using Depth Anything~\cite{depthanything} and Segment Anything~\cite{kirillov2023segment} for the image from COCO Dataset with 2D box labels. }
    \label{fig: monodepth}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/pcd.pdf}
    \caption{\textbf{Prediction with 2D prompt and point cloud.} We ran Gaussian Splatting~\cite{kerbl20233d} on scene \textit{sculpture} from nerfstudio dataset~\cite{nerfstudio} to obtain the point cloud. The 2D prompt is obtained from human annotation.}
    \label{fig: pcd}
\end{figure}



% Another potential application of our model is to assist human annotators in creating new datasets for 3D detection. Since our model can generate multiple predictions for an object, the annotation process can be streamlined. Instead of creating a box from scratch and making adjustments manually, annotators can simply select the best box from the candidates generated by our model and make further refinements using the diffusion process.














==> sec/07_ack.tex <==
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2024/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.

==> sec/08_ref.tex <==
\clearpage


\begin{small}

\bibliographystyle{ieeenat_fullname}
\bibliography{bib}

\end{small}


==> sec_/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec_/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec_/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec_/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
